On the Complexity of Instationary Gas Flows

We study a simplistic model of instationary gas flows consisting of a sequence of k stationary gas flows. We present efficiently solvable cases and NP-hardness results, establishing complexity gaps between stationary and instationary gas flows (already for k=2) as well as between instationary gas s-t-flows and instationary gas b-flows.

==> setup-preprint.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Packages
\usepackage[american]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{amsmath,amssymb,amsthm}
%\usepackage[pdftex]{graphicx}
\usepackage{booktabs}
\usepackage{enumitem}
\usepackage[binary-units=true]{siunitx}
\usepackage{url}
\usepackage{xspace}
\usepackage{relsize}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{todonotes}
\usepackage{pgfplots}

\usepackage{tikz}
\usepackage{csquotes}
% Anpassung der Laufweiten für Buchstaben,
% um bessere Umbrüche zu erreichen.
% Siehe: Das LaTeX2e-Sündenregister
\usepackage{microtype}
\usepackage{notationForne}

\usepackage[colorlinks,citecolor=blue,linkcolor=blue]{hyperref} % should always be the last package


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Modify text style of title and authors
\makeatletter
\patchcmd{\@settitle}{\uppercasenonmath\@title}{\scshape\large}{}{}
\patchcmd{\@setauthors}{\MakeUppercase}{\scshape\normalsize}{}{}
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Re-definitions of the algorithm2e package
\renewcommand{\algorithmcfname}{Algorithm}
\renewcommand*{\listalgorithmcfname}{List of Algorithms}
\SetArgSty{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Moderate Anpassung der Parameter, die TeX bei der
% Berechnung von Zeilenumbrüchen verwendet.
% Siehe: Das LaTeX2e-Sündenregister
\tolerance 1414
\hbadness 1414
\emergencystretch 1.5em
\hfuzz 0.3pt
\widowpenalty=10000
\vfuzz \hfuzz
\raggedbottom


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AMS theorem standard setup
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{assumption}{Assumption}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% special biblatex eprint styles
\DeclareFieldFormat{eprint:urn}{%
  URN\addcolon\space
  \ifhyperref
    {\href{http://www.nbn-resolving.org/#1}{\nolinkurl{#1}}}
    {\nolinkurl{#1}}}

\DeclareFieldFormat{eprint:optonline}{%
  Optimization Online\addcolon\space
  \ifhyperref
    {\href{http://www.optimization-online.org/DB_HTML/#1.html}{\nolinkurl{#1}}}
    {\nolinkurl{#1}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% TikZ externalize setup
\usetikzlibrary{external}

\tikzexternalize{InstationaryGasFlows} % provide the file~s real name
\newcommand{\includetikz}[1]{%
  \tikzexternalenable
  \tikzsetnextfilename{#1}
  \input{#1.tikz}
  \tikzexternaldisable
}

\tikzexternaldisable



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "gas-trans-hardness_preprint"
%%% End:

